Generalization of Siegel's Method to theta 1

We present a new proof of the transformation law of $\vartheta_1$ under the action of the generator of the full modular group $\Gamma$ using Siegel's method.

==> cover_letter.tex <==
Ramanujan Journal.
Dear Dr. Ken Ono,
We, Maher and Ali, were trying to provide a general approach or proof to all the transformation laws of the four Jacobi theta functions
In our paper we present a new proof of the generalized transformation law of these theta functions. Our proof was originally inspired by Basil Gordon’s proof of the transformation law of the Dedekind eta function. We generalize his proof for 2 variables and for all theta functions, where our proof is shorter and lighter than previously addressed proofs. Since most previous papers provide proofs of the transformation law for specific matrices like the inversion or the generators. We extend that to all matrices in full modular group and Γ(2).
We confirm that this paper has not been published before. Both authors have approved the manuscript and the submission to Ramanujan’s Journal.
Yours sincerely.
